Binary expression of ancestors in the Collatz graph

The Collatz graph is a directed graph with natural number nodes and where there is an edge from node $x$ to node $T(x)=T_0(x)=x/2$ if $x$ is even, or to node $T(x)=T_1(x)=\frac{3x+1}{2}$ if $x$ is odd. Studying the Collatz graph in binary reveals complex message passing behaviors based on carry propagation which seem to capture the essential dynamics and complexity of the Collatz process. We study the set $\mathcal{E} \text{Pred}_k(x)$ that contains the binary expression of any ancestor $y$ that reaches $x$ with a limited budget of $k$ applications of $T_1$. The set $\mathcal{E} \text{Pred}_k(x)$ is known to be regular, Shallit and Wilson [EATCS 1992]. In this paper, we find that the geometry of the Collatz graph naturally leads to the construction of a regular expression, $\texttt{reg}_k(x)$, which defines $\mathcal{E} \text{Pred}_k(x)$. Our construction, is exponential in $k$ which improves upon the doubly exponentially construction of Shallit and Wilson. Furthermore, our result generalises Colussi's work on the $x = 1$ case [TCS 2011] to any natural number $x$, and gives mathematical and algorithmic tools for further exploration of the Collatz graph in binary.

==> decode.tex <==
\section{Decoding $\E(p)$}\label{app:decode}

In this Section, we prove the remaining points of Corollary~\ref{cor:decode} (Section~\ref{sec:begin}). In order to prove Points 5 and 6, we will need results from Section~\ref{sec:end}.

\paragraph{Corollary~\ref{cor:decode}}
We have the following for all $n\in\N$:

% \begin{center}
% \begin{align*}
% \E^{-1}(\texttt{0}^n) &= \; \downarrow^n\\
% \E^{-1}(\texttt{1}(\texttt{0})^n) &= \; \downarrow^n \leftarrow\\
% \E^{-1}(\texttt{1}(\texttt{0}^{2n})\texttt{1}) &= \; \leftarrow (\downarrow\leftarrow)^{n} \leftarrow \\
% \E^{-1}(\texttt{1}(\texttt{0}^{2n+1})\texttt{1}) &= \; (\leftarrow\downarrow)^{n+1}\downarrow\\
% \E^{-1}((\texttt{01})^{n+1}) &= \; \leftarrow \downarrow (\downarrow)^{2n}\\
% \E^{-1}(\texttt{1}^n) &= \; \leftarrow^n\\
% \end{align*}
% \end{center}

\begin{enumerate}
\item $\E^{-1}(\texttt{0}^n) = \; (\downarrow)^n$
\item $\E^{-1}(\texttt{1}(\texttt{0})^n) = \; (\downarrow)^n \leftarrow$
\item $\E^{-1}(\texttt{1}(\texttt{0})^{2n}\texttt{1}) = \; \leftarrow (\downarrow\leftarrow)^{n} \leftarrow$
\item $\E^{-1}(\texttt{1}(\texttt{0})^{2n+1}\texttt{1}) = \; (\leftarrow\downarrow)^{n+1}\downarrow$
\item $\E^{-1}((\texttt{01})^{n+1}) = \; \leftarrow \downarrow (\downarrow)^{2n}$
\item $\E^{-1}(\texttt{1}^n) = \; (\leftarrow)^n$
\end{enumerate}

Note that these statements allow to predict the first $\lfloor \text{log}_2(x) \rfloor + 1$ arrows of the parity vector taken along the Collatz sequence of any $x\in\N$ of which binary representation matches one of the different given expressions.

\begin{proof}

\begin{enumerate}

\item Proved in main text
\item By Theorem~\ref{th:begin}, we know that $\E((\downarrow)^n \leftarrow) = b \bullet \E((\downarrow)^n)$ with $b\in\{\texttt{0},\texttt{1}\}$. From Point~\ref{point:dec1} of this Corollary we have $\E((\downarrow)^n) = \texttt{0}^n$ and from the proof of this Point we know that $\alpha_{0,-1}((\downarrow)^n) = 0$. Since the arrow $\leftarrow$ is not admissible for $0$ we conclude $b=\texttt{1}$ and $\E((\downarrow)^n \leftarrow) = \texttt{1}(\texttt{0})^n$ and we have the result.

\item We show by induction on $n$ that, for $p_n = \; \leftarrow (\downarrow\leftarrow)^{n}$ we have $\E(p_n)=\texttt{1}(\texttt{0})^{2n}$ and $\alpha_{0,-1}(p_n) = 2$. For $n=0$, $p_0 = \;\leftarrow$, we know that $\alpha_{0}(\leftarrow) = (1,2)$ since $1$ is the smallest integer on which $T_1$ can be applied. Hence, $\E(p_0) = \I^{-1}_1(\alpha_{0,0}(p_0)) = \I^{-1}_1(1) = \texttt{1}$ and $\alpha_{0,-1}(p_0) = 2$. Let suppose the result true for some $n\in\N$. By Theorem~\ref{th:begin}, we have $\E(p_{n+1}) = \E(\composeP{\composeP{p_{n}}{\downarrow}}{\leftarrow}) = b_2 b_1 \bullet \E(p_n) $ with $b_1,b_2\in\{\texttt{0},\texttt{1}\}$. We know that $b_1 = \texttt{0}$ since $\alpha_{0,-1}(p_n) = 2$ and $b_1$ corresponds to the arrow $\downarrow$. Now, by admissibility of $\downarrow$, we have $\alpha_{0,-1}(\composeP{p_{n}}{\downarrow}) = T(\alpha_{0,-1}(p_n)) = T(2) = 1$. Hence we have $b_2 = \texttt{0}$ because $\leftarrow$ is admissible for $1$. By the same argument, we have $\alpha_{0,-1}(\composeP{\composeP{p_{n}}{\downarrow}}{\leftarrow}) = T(\alpha_{0,-1}(\composeP{p_{n}}{\downarrow})) = T(1) = 2$ and we conclude $\E(p_{n+1})=\texttt{1}(\texttt{0})^{2(n+1)}$ and $\alpha_{0,-1}(p_{n+1}) = 2$ and the induction is proved. Now, we know that $\E(\leftarrow (\downarrow\leftarrow)^{n} \leftarrow) = \texttt{1}\bullet\E(\leftarrow (\downarrow\leftarrow)^{n})=\texttt{1}\bullet\E(p_n)$ because $\leftarrow$ is not admissible for $\alpha_{0,-1}(p_n) = 2$. Hence we have the result.

\item Very similar to Point 3.

\item By induction, for $p_n=\;\leftarrow \downarrow (\downarrow)^{2n}$, let's prove $\E(p_n) = (\texttt{01})^{n+1}$ and $\alpha_{0,-1}(p_n) = 1$.  For $n=0$, we have $\E(\leftarrow\downarrow) = \texttt{0} \bullet \E(\leftarrow) = \texttt{01}$ since $\downarrow$ is admissible for $2 = \alpha_{0,-1}(\leftarrow)$ and $\E(\leftarrow) = \texttt{1}$. By Theorem~\ref{th:end}, $\alpha_{0,-1}(p_0) = T_{0,1}(\alpha_{0,-1}(\leftarrow)) = T_{0,1}(2) = 1$.

Now, $\E(\leftarrow \downarrow (\downarrow)^{2(n+1)}) = b_2 b_1 \bullet\E(\leftarrow \downarrow (\downarrow)^{2n})$. We have $b_1=\texttt{1}$ since $\downarrow$ is not admissible for $\alpha_{0,-1}(p_n)=1$. By Theorem~\ref{th:end}, $\alpha_{0,-1}(\composeP{p_n}{\downarrow}) = T_{0,1}(\alpha_{0,-1}(p_n)) = T_{0,1}(1) = 2$. Hence $b_0=\texttt{0}$ since $\downarrow$ is admissible for $2$. Hence we have $\E(p_{n+1}) = \texttt{01}(\texttt{01})^{n+1} = (\texttt{01})^{n+2}$ which gives the result.

\item Let's have $p_n = (\leftarrow)^n$. We have $\E(p_0) = \eta$. For $n\geq1$, by Lemma~\ref{lem:left}, we know that $\alpha_{0,-1}(p_n) = 3^n - 1$ which is always even. Hence, $\E(p_{n+1}) = \E(\composeP{p_n}{\leftarrow}) = \texttt{1} \bullet \E(p_n) = (\texttt{1})^{n+1}$ since the arrow $\leftarrow$ is never admissible for an even number.

\end{enumerate}
\end{proof}

==> figures/poles.tex <==

\begin{figure}[h!]

\centering
\begin{BVerbatim}
p=[1,1,0,0]

x=3
11
101
1

x=227
111000*11
101010*101
1

x=14563
111000111000*11
101010101010*101
1

x=932067
111000111000111000*11
101010101010101010*101
1
\end{BVerbatim}
\caption{First four OCS occurrences of the path \texttt{[1,1,0,0]} on the pole $1$ }\label{fig:pole1}
\end{figure}

\begin{figure}[h!]
    \centering
                \begin{BVerbatim}
p=[1, 0, 1, 1, 0, 1]

x=6949999424953
1100101001000101100001111110011010110111001
1001011110110100001001011110110100001001011
1110001110001110001110001110001110001110001
1010101010101010101010101010101010101010101
1

x=125200059281800434715723773369
110010100100010110000111111001101011011101001111000000*1100101001000101100001111110011010110111001
100101111011010000100101111011010000100101111011010000*1001011110110100001001011110110100001001011
111000111000111000111000111000111000111000111000111000*1110001110001110001110001110001110001110001
101010101010101010101010101010101010101010101010101010*1010101010101010101010101010101010101010101
1
\end{BVerbatim}

    \caption{First two OCS occurrences of the path \texttt{[1, 0, 1, 1, 0, 1]} on the pole $1$}\label{fig:pole2}
\end{figure}


\begin{figure}[h!]
    \centering
\begin{BVerbatim}
p=[1, 1, 1, 1, 0, 0]

x=1346319
101001000101100001111
111101101000010010111
1011100011100011100011
10001010101010101010101
1101
101
1

x=24253141442886079122191
101001000101100001111110011010110111010011110000001100*101001000101100001111
111101101000010010111101101000010010111101101000010010*111101101000010010111
10111000*111000111000111000111000111000111000111000111000111000*11100011100011
10001010101010101010101010101010101010101010101010101010101010101010101010101
1101
101
1
\end{BVerbatim}

\caption{First two OCS occurrences of the path \texttt{[1, 1, 1, 1, 0, 0]} on the pole $13$ (\texttt{1101})}\label{fig:pole3}
\end{figure}

==> figuresapp.tex <==
\section{Additional Figures}\label{app:figures}

%\input{figures/G_s_}
%\input{figures/path_gene}
%\input{figures/poles2.tex}


==> proofs.tex <==
\section{Proofs}\label{app:proofs}
This Appendix presents the proofs that were omitted in the main body.
\lembij*
\begin{proof}
By cardinality, because $|\Pa_n| = |\{0,\ldots,2^n-1\}| = 2^n$, we just have to prove the injectivity of $f$. Let $p_1,p_2\in\Pa_n$ such that $f(p_1)=f(p_2)$. We write $p_1 = a_0 \cdot \ldots \cdot a_{n-1}$ and $p_2 = a'_0 \cdot \ldots \cdot a'_{n-1}$ with $a_i,a'_i\in\{\downarrow,\leftarrow\}$. Since $\alpha_{0,0}(p_1) = \alpha_{0,0}(p_2)$ and that the Collatz process is deterministic we deduce:
\begin{align*}
\alpha_{0,0}(p_1) &= \alpha_{0,0}(p_2)\\
\alpha_{0,1}(p_1) &= \alpha_{0,1}(p_2)\\
&\vdots\\
\alpha_{0,-1}(p_1) &= \alpha_{0,-1}(p_2)
\end{align*}
Thus, by Definition~\ref{def:occ} we deduce that $a_{i} = a'_{i}$ for $0 \leq i < n$. Thus $p_1=p_2$ which ends the proof.
\end{proof}

\thend*
\begin{proof}
Since any $x\in\N$ is an occurrence of the parity vector $\epsilon$, we have $\alpha_{0}(\epsilon) = (0,)$ (tuple with one element). Hence $\alpha_{0,-1}(\epsilon) = \alpha_{0,\norm{\epsilon}}(\epsilon) = \alpha_{0,0}(\epsilon) = 0$. Now, let $p\in\Pa_n$ for some $n\in\N$ and $k = l(p)$. Then notice that Equations~(\ref{eq:down}) and (\ref{eq:up}) are well defined because of Theorem~\ref{th:struct_occ}. Indeed, we know that $\alpha_{0,-1}(p) < 3^{l(p)} = 3^k$ thus $\alpha_{0,-1}(p)\in\ZnZ{3^k}$ and $\alpha_{0,-1}(p)\in\ZnZ{3^{k+1}}$ and we can use the operators $T_{0,k}$ and $T_{0,k+1}$ on it. 
\\
Let's consider $\alpha_{0,-1}(\composeP{p}{a})$ with $a\in\{\downarrow,\leftarrow\}$. Two cases:
\begin{itemize}
\item The arrow $a$ is admissible for $\alpha_{0,-1}(p)$: in that case, by Lemma~\ref{lem:undeux}, we know that $(\alpha_{0,0}(\composeP{p}{a}), \alpha_{0,1}(\composeP{p}{a}), \ldots, \alpha_{0,\norm{p}}(\composeP{p}{a}))$ is the first occurrence of $p$. Hence, $\alpha_{0,-1}(p) = \alpha_{0,\norm{p}}(\composeP{p}{a})$ and we have $\alpha_{0,-1}(\composeP{p}{a}) = T(\alpha_{0,\norm{p}}(\composeP{p}{a})) = T(\alpha_{0,-1}(p)) = T_{i}(\alpha_{0,-1}(p))$. With $i=0$ if $a=\;\downarrow$ or $i=1$ if $a=\;\leftarrow$. Then two cases:
\begin{enumerate} 
  \item If $a=\;\downarrow$ then $\alpha_{0,-1}(p)$ is even and $\alpha_{0,-1}(\composeP{p}{a}) = T_0(\alpha_{0,-1}(p)) = T_{0,k}(\alpha_{0,-1}(p))$  by Appendix~\ref{app:structT}, Lemma~\ref{lem:t0}.
  \item If $a=\;\leftarrow$ then $\alpha_{0,-1}(p)$ is odd and $\alpha_{0,-1}(\composeP{p}{a}) = T_1(\alpha_{0,-1}(p)) = T_{1,k+1}(\alpha_{0,-1}(p))$  by Appendix~\ref{app:structT}, Lemma~\ref{lem:t1}.
\end{enumerate}
 \item The arrow $a$ is not admissible for $\alpha_{0,-1}(p)$: in that case, by Lemma~\ref{lem:undeux}, we know that $(\alpha_{0,0}(\composeP{p}{a}), \alpha_{0,1}(\composeP{p}{a}), \ldots, \alpha_{0,\norm{p}}(\composeP{p}{a}))$ is the second occurrence of $p$. Hence, by Theorem~\ref{th:struct_occ}, $\alpha_{0,\norm{p}}(\composeP{p}{a}) = 3^k + \alpha_{0,-1}(p)$. Now, $\alpha_{0,-1}(\composeP{p}{a}) = T(\alpha_{0,\norm{p}}(\composeP{p}{a})) = T(3^k + \alpha_{0,-1}(p))$. Then two cases:
\begin{enumerate} 
  \item If $a=\;\downarrow$ then $\alpha_{0,-1}(p)$ is odd and $\alpha_{0,-1}(\composeP{p}{a}) = T_0(3^k + \alpha_{0,-1}(p)) = \frac{3^k + \alpha_{0,-1}(p)}{2} = T_{0,k}(\alpha_{0,-1}(p))$ by Appendix~\ref{app:structT}, Lemma~\ref{lem:t0}.
  \item If $a=\;\leftarrow$ then $\alpha_{0,-1}(p)$ is even and $\alpha_{0,-1}(\composeP{p}{a}) = T_1(3^k + \alpha_{0,-1}(p)) = \frac{3^{k+1} + 3\alpha_{0,-1}(p) +1}{2} = T_{1,k}(\alpha_{0,-1}(p))$ by Appendix~\ref{app:structT}, Lemma~\ref{lem:t1}.
\end{enumerate}
\end{itemize}
In all the cases we get the result.
\end{proof}
\lembijg*
\begin{proof}
\begin{enumerate}
\item The function $g$ is well defined. Indeed, for any $\omega\in\E\Predk{x}$ \label{point:lembijg1}
\begin{align*}
\omega \in \E\Predk{x} &\Leftrightarrow \exists p \in \Pa \; \I(\omega) = 2^{\norm{p}}i + \I(\E(p)) \text{ with } \alpha_{0,-1}(p) = x \text{ mod } 3^k \text{ and } l(p) = k\\
& \Leftrightarrow \I(\omega) = 2^{\norm{p}}i + \alpha_{0,0}(p) \\
& \Leftrightarrow \I(\omega) = \alpha_{i,0}(p) = g(\omega) \in \Predk{x}
\end{align*}
With $i = \lfloor \frac{x}{3^k} \rfloor$.
\item The function $g$ is injective. Let $\omega_1,\omega_2\in\E\Predk{x}$ with $\omega_1 = \omega\bullet\E(p_1)$ and $\omega_2 = \omega\bullet\E(p_2)$ with $\omega=\eta$ if $i=\lfloor \frac{x}{3^k} \rfloor=0$ else $\omega=\I^{-1}(i)$. We have $x=\alpha_{i,-1}(p_1) = \alpha_{i,-1}(p_2)$ by hypothesis. Suppose $g(\omega_1) = g(\omega_2)$. We get $2^{\norm{p_1}}i + \I(\E(p_1)) = 2^{\norm{p_2}}i + \I(\E(p_2))$. Hence, $2^{\norm{p_1}}i + \alpha_{0,0}(p_1) = 2^{\norm{p_2}}i + \alpha_{0,0}(p_2)$. By Theorem~\ref{th:struct_occ} we get $\alpha_{i,0}(p_1) = \alpha_{i,0}(p_2)$. If $\norm{p_1} \neq \norm{p_2}$, for instance $\norm{p_1} < \norm{p_2}$ we have $p_2 = \composeP{p_1}{(\downarrow)^{\norm{p_2}-\norm{p_1}}}$. Indeed, by determinism of the Collatz process, $p_1$ must be a prefix of $p_2$ as they both are forward feasible for $y = \alpha_{i,0}(p_1) = \alpha_{i,0}(p_2)$. Furthermore, we can't add any more arrows of type $\leftarrow$ because $l(p_1)=l(p_2)$. But, $\alpha_{i,-1}(p_1) = x \neq 0$ thus $\alpha_{i,-1}(p_2) = x/(2^{\norm{p_2}-\norm{p_1}}) \neq x$ which contradicts $\alpha_{i,-1}(p_1)=\alpha_{i,-1}(p_2)$. Hence we have $\norm{p_1}=\norm{p_2}$ and thus $p_1=p_2$ because, by determinism of the Collatz process, there is only one path of a given norm between $\alpha_{i,0}(p_1)$ and $\alpha_{i,-1}(p_1)$ and thus one corresponding parity vector. Hence, $\omega_1 = \omega_2$.
\item The function $g$ is surjective. Let $y\in\Predk{x}$. There exists $p\in\Pa$ with $\alpha_{i,0} = y$ and $\alpha_{i,-1} = x$ with $i = \lfloor \frac{x}{3^k} \rfloor$. Similarly to the proof of Point~\ref{point:lembijg1}, the reader can verify that $\E(p)\in\E\Predk{x}$ is a valid antecedent of $y$ in the case $i=0$ and that $\I^{-1}(i)\bullet\E(p)\in\E\Predk{x}$ is a valid antecedent of $y$ otherwise.
\end{enumerate}
\end{proof}
% % We first prove surjectivity, two cases:

% % \begin{itemize}

% % \item If $x < 3^k$ then, by Lemma~\ref{lem:better_pred} we know that $\Predk{x} = \{ y \in\N \; | \; \exists p \in \Pa \quad \alpha_{0,0}(p) = y \text{ and } \alpha_{0,-1}(p) = x \text{ and } l(p) = k  \}$. Let $y\in\Predk{x}$, we have $\alpha_{0,0}(p) = y$ for some $p\in\Pa$. We have $\E(p) \in \E\Predk{x}$ because $\alpha_{0,-1}(p) = x \text{ and } l(p) = k$. Furthermore, by Lemma~\ref{lem:shortlem} we have $\I(\E(p)) = y$. Hence, $f(\E(p)) = y$ and the function $f$ is surjective in that case. 

% % \item If $x \geq 3^k$ then, by Lemma~\ref{lem:better_pred} we know that $\Predk{x} = \{ y \in\N \; | \; \exists p \in \Pa \quad \alpha_{i,0}(p) = y \text{ and } \alpha_{i,-1}(p) = x \text{ and } l(p) = k  \}$ with $i = \lfloor \frac{x}{3^k} \rfloor $. Let $y\in\Predk{x}$, by Theorem~\ref{th:struct_occ} we have $\alpha_{i,0}(p) = y = 2^{\norm{p}}i + \alpha_{0,0}(p)$ for some $p\in\Pa$. We have $\I^{-1}(i)\bullet\E(p) \in \E\Predk{x}$ because $\alpha_{i,-1}(p) = x \text{ and } l(p) = k$. Furthermore, we have $\I(\I^{-1}(i)\bullet\E(p)) = 2^{\norm{p}}i + \I(\E(p))  = 2^{\norm{p}}i + \alpha_{0,0}(p) = y $ by Lemma~\ref{lem:shortlem}. Hence, $f(\I^{-1}(i)\bullet\E(p)) = y$ and $f$ is surjective in that case.



% % \end{itemize}



% \end{proof}

\lemdown*
\begin{proof}

We have $l(p_n) = l(p) = k > 0$. By Lemma~\ref{lem:star}, we know that $\alpha_{0,-1}(p)\in(\ZnZ{3^k})^*$. Furthermore, by Theorem~\ref{th:end}, $\alpha_{0,-1}(p_n) = T^{n\pi_k}_{0,k}(\alpha_{0,-1}(p)) = (2^{-n}_k)^{\pi_k} \alpha_{0,-1}(p) =  1*\alpha_{0,-1}(p) = \alpha_{0,-1}(p)$ since $\pi_k$ is the order of the group $(\ZnZ{3^k})^*$. Hence we have $p_n \simeq_k p$. Furthermore, by Theorem~\ref{th:begin} we know that $\E(p_{n+1}) = \omega \bullet \E(p_{n})$ with $\omega=b_0\ldots b_{\pi_k - 1} \in\Bs$ with $|\omega| = \pi_k$ such that:
$$ b_{\pi_k - 1 - i } = \begin{cases} \texttt{0} &\text{ if } 2^{-i_0 - i}_k \text{ is even}\\\texttt{1} &\text{ if } 2^{-i_0 - i}_k \text{ is odd}\end{cases}$$
With $0 \leq i_0 < \pi_k$ such that $\alpha_{0,-1}(p) = 2^{-i_0}_{k}$ in $(\ZnZ{3^k})^{*}$. By definition, the string $\omega=b_0\ldots b_{\pi_k - 1}$ is exactly $\R{i_0}{\Pi_k}$ and we have the result.

\end{proof}



% \correallife*
% \begin{proof}

% The result without the bound on $n$ is an immediate consequence of Theorem~\ref{th:main}:

% If $x=0$, $y \in \Predk{x} \Leftrightarrow k = 0 \text{ and } y = 0 \Leftrightarrow \exists n\in\N \; \texttt{0}^n \bullet \I^{-1}(y) \text{ is recognised by } \reg{0}{0} = (\texttt{0})^* $ since any $n\in\N$ will work.

% If $x\neq0$, by Lemma~\ref{lem:bijg}, we have:
% $$ y \in \Predk{x} \Leftrightarrow g^{-1}(y) \in \E\Predk{x} \Leftrightarrow g^{-1}(y) \text{ is recognised by } \regk{x}$$

% We have $g^{-1}(y)=\omega\in\Bs$ such that $\I(\omega) = y$. Hence, there exists $n\in\N$ such that $g^{-1}(y)  =  \texttt{0}^n \bullet \I^{-1}(y)$ and we get the result without the bound on $n$.

% The stake is now to bound $n$, the number of leading $\texttt{0}$s one has to prepend to the binary representation of $y$ in order to test whether $y\in\Predk{x}$. We derive this bound from analysing $\regk{x}$ hence we review all the cases of the proof of Theorem~\ref{th:main}.

% Let $x\in\N$. Suppose $x$ is a multiple of 3. If $x=0$ we have $\reg{0}{0} = (0)^{*}$ and $\Pred{0}{0} = \{0\}$ hence any bound will work. If $k > 1$ we have $\reg{k}{x} = \emptyset$ hence any bound will also work. When $k=0$ and $x\neq 0$, we have $\reg{0}{x} = (\I^{-1}(x))(\texttt{0})^{*}$ thus $\reg{0}{x}$ starts with a bit equal to $\texttt{1}$ hence it will not match any leading $\texttt{0}$ and taking $B(x,k)=0$ will work (we are in a special case of $x\geq3^k$).

% Suppose that $x$ is not a multiple of 3. If $x\geq3^k$ we have $\reg{k}{x} = (\I^{-1}(\lfloor \frac{x}{3^k} \rfloor ))(\reg{k}{(x \text{ mod } 3^k)})$, again, $\reg{k}{x}$  starts with a bit equal to $\texttt{1}$ and the bounde $B(x,k)=0$ will work.

% Now, the last case is $x\in(\ZnZ{3^k})^*$ with $k>0$. We prove by induction on $k>0$ the following result:


%  $$\tilde{H}(k) = ``\forall x\in(\ZnZ{3^k})^*,\, \text{the number of leading } \texttt{0} \text{s that } \regk{x} \text{ can accept is bounded by } (k+1)^{2}  "$$

% \textbf{Base $k=1$.} In that case we only have $x=1$ and $x=2$ to consider. We have:
% \begin{align*}
% \reg{1}{1} &= \texttt{(01)*(((0)(1)((0)*)))}\\
% \reg{1}{2} &= \texttt{(10)*((()(1)((0)*)))}
% \end{align*}

% In both case the maximum number of leading \texttt{0}s that can be accepted is bounded by $1 \leq (1+1)^2 = 4$ hence the bound $\B(x,k) = (k+1)^2$ is valid.\\

% \noindent \textbf{Inductive step.} Suppose the result true for some $k > 0$. By Theorem~\ref{th:main} we have:
% \begin{align*} \reg{k+1}{x} = (\R{i_0}{\Pi_{k+1}})^*( \quad &(\join_0) \; (b_0) \; (\reg{k}{2^{-0}_{k}}) \quad |\\
%                                              &(\join_1) \; (b_1) \; (\reg{k}{2^{-1}_{k}}) \quad |\\
%                                              &(\join_2) \; (b_2) \; (\reg{k}{2^{-2}_{k}}) \quad |\\
%                                              &\quad\quad\vdots\\
%                                              &(\join_{\pi_k-1}) \; (b_{\pi_k-1}) \; (\reg{k}{2^{-(\pi_k-1)}_{k}}) \quad ) \end{align*}

%  The longest trail of consecutive \texttt{0}s in the string $\Pi_{k+1}$ (and thus in $\R{i_0}{\Pi_{k+1}}$) will correspond to the \texttt{0s} given by the parity of the sequence $2^m, 2^{m-1}, \dots, 2^{1}$ with $m$ the largest integer such that $2^m < 3^{k+1}$. We have $m = \lfloor (k+1)\text{log}_2(3) \rfloor$.  The same is true for the maximum number of leading $\texttt{0}$s in the expression $\join_{i_2}$. The bit $b_{i_2}$ can also be equal to $\texttt{0}s$. Let's call $z_{k+1}$ (resp. $z_k$) the number of leading $\texttt{0}$s that $\reg{k+1}{x}$ (resp. $\reg{k}{x}$) can accept. Since $\R{i_0}{\Pi_{k+1}}$ is not all \texttt{0}s, we can't use Kleene star to have an unbounded number of leading \texttt{0}s. We deduce: $z_{k+1} \leq \text{max}((k+1)\text{log}_2(3), (k+1)\text{log}_2(3) + 1 + z_k) \leq 2(k+1) + 1 + z_k$. By induction hypothesis we deduce, $z_{k+1} \leq 2(k+1) + 1 + (k+1)^2 = (k+2)^2  $.


% Hence we have the result and the bound $B(x,k) = (k+1)^2$ is valid when $x < 3^k$.

% % The goal is to find a bound on the number of leading $\texttt{0}s$ this expression can accept. The longest trail of consecutive \texttt{0}s is $\Pi_k$ will correspond to the parity of the sequence $2^m, 2^{m-1}, \dots, 2^{1}$ with $m$ the largest integer such that $2^m < 3^k$. We have $m = \lfloor k\text{log}_2(3) \rfloor$. The same is true for the maximum number of leading \texttt{0}s in the expression $\join_{i_2}$. Since the bit $b_0$ can also be equal to $\texttt{0}s$ we deduce as an upper bound $\sum_{m=0}^{k} (m\text{log}_2(3) + 1) = \frac{k(k+1)}{2}\text{log}_2(3) + (k+1) = (k+1)( \frac{k\text{log}_2(3) + 2}{2}) \leq (k+1)^2 = B(x,k)$.


% %If $x$ is a multiple of three and $k>0$ the result is obvious since any bound will work as $\regk{x} = \eta$ and $\Predk{x} = \emptyset$, no words are recognised in that case. Similarly, if $k=0$ and $x=0$, the result is the same as in the unbounded case, any bound will do. If $x\geq 3^k$ not a multiple of three we have $\reg{k}{x} = \I^{-1}( \lfloor \frac{x}{3^k} \rfloor ) \bullet \reg{k}{(x\text{ mod } 3^k)}$ thus the regular expression starts with a $\texttt{1}$ and there is no need for leading \texttt{0}s thus the bound $B(x,k)=0$.

% \end{proof}
